KNIFE: Distilling Reasoning Knowledge From Free-Text Rationales

Language models (LMs) have yielded impressive results on many language reasoning tasks, but their unexpected errors raise doubts about their reasoning abilities. In light of this, there is growing interest in finetuning/prompting LMs with both task instances and their associated free-text rationales (FTRs), which explain the correct reasoning process for predicting the correct task output (i.e., how to be "right for the right reasons"). However, existing finetuning methods fail to improve LM performance, while prompting needs prohibitively large (i.e., >50B) LMs to work well. We propose KNIFE, which shows that reasoning knowledge can be effectively distilled from FTRs into a small (i.e., <1B) LM and improve the LM's performance. First, KNIFE finetunes a teacher LM (given task input and FTR) to predict the task output, transferring reasoning knowledge from the FTRs to the teacher's hidden states. Second, KNIFE finetunes a student LM (given task input only) such that its hidden states are aligned with the teacher's. Thus, the student is endowed with reasoning knowledge but can be used for inference without direct FTR input. On two question-answering datasets, KNIFE outperforms various finetuning and prompting baselines in fully-supervised and low-resource settings. Also, we observe that FTR quality is crucial to KNIFE's performance.

==> sections/6_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

The major limitations of this work are as follows: (1)~Due to limited computational resources, we only conduct experiments on small models. In the future, we will explore the performance of \method~on large-scale models. (2)~Our study is limited to encoder-decoder transformer architectures (\eg T5). It is interesting to extend \method~to decoder-only (\eg GPT) and encoder-only (\eg BERT) architecture, especially to apply the bottleneck design to other attention mechanisms besides cross-attention. (3)~\method~requires each training instance to be accompanied by an FTR. In the real world, however, it is common to only have FTRs for a subset of training instances. We leave applying \method~to such settings for future work.

==> sections/8_conclusion.tex <==
\section{Conclusion}
% In this paper, we propose \method~to improve model performance by learning from free-text rationales.
% Unlike previous works, \method~circumvents input distribution shift, conflicting training objectives, and the necessity for large LMs.
% We hope our work can facilitate and inspire future research in the explanation-based learning area.

==> sections/9_ethicsstatement.tex <==
\section{Broader Impacts}
Regarding ethical concerns, all datasets used in this work are publicly available. Our method makes use of large language models to generate free-text rationales. We are aware that the resulting rationales may contain social biases. Such biases may be further inherited by the student model. 
